Cannings models, population size changes and multiple-merger coalescents

Multiple-merger coalescents, e.g. $\Lambda$-$n$-coalescents, have been proposed as models of the genealogy of $n$ sampled individuals for a range of populations whose genealogical structures are not captured well by Kingman's $n$-coalescent. $\Lambda$-$n$-coalescents can be seen as the limit process of the discrete genealogies of Cannings models with fixed population size, when time is rescaled and population size $N\to\infty$. As established for Kingman's $n$-coalescent, moderate population size fluctuations in the discrete population model should be reflected by a time-change of the limit coalescent. For $\Lambda$-$n$-coalescents, this has been explicitly shown for only a limited subclass of $\Lambda$-$n$-coalescents and exponentially growing populations. This article gives a general construction of time-changed $\Lambda$-$n$-coalescents as limits of specific Cannings models with rather arbitrary time changes.

==> main.tex <==

\section{Introduction}\label{sec:intro}
The genealogies of samples from populations with highly variant offspring numbers, for instance due to sweepstake reproduction or rapid selection, are not well modelled by Kingman's $n$-coalescent. As a more realistic alternative, multiple-merger coalescents, especially $\Lambda$-coalescents have been proposed, as reviewed in \cite{Tellier2014}, \cite{irwin2016importance} and \cite{eldon2016current}. $\Lambda$-$n$-coalescents, introduced by \cite{Pitman1999,Sagitov1999,donnelly1999particle}, are Markovian processes $(\Pi_t)_{t\geq 0}$, which describe the genealogy of a set of individuals $\{1,\ldots,n\}$. This is done by representing the ancestral lineages present at time $t$ of these individuals by the sets of offspring of each ancestral lineage in the sample. Thus, $(\Pi_t)_{t\geq 0}$ can be defined as a random process with states in the set of partitions of $\{1,\ldots,n\}$ and transitions via merging of blocks (i.e. merging of ancestral lineages to a common ancestor). For a $\Lambda$-$n$-coalescent, the infinitesimal rates of any merger of $k$ of $b$ present lineages is given by $\lambda_{b,k}:=\int_0^1 x^{k-2}(1-x)^{b-k}\Lambda(dx)$, where $\Lambda$ is a finite measure on $[0,1]$. This includes Kingman's $n$-coalescent if $\Lambda$ is the Dirac measure in 0.\\ As in the case of Kingman's $n$-coalescent being the limit genealogy from samples taken from a discrete Wright-Fisher or Moran model, $\Lambda$-$n$-coalescents can be constructed as the (weak) limit of genealogies from samples of size $n$ taken from Cannings models. The limit is reached as population size $N$ goes to infinity and time is rescaled, see \cite{Moehle2001}. Time is rescaled by using $\lceil c^{-1}_N\rceil$ generations in the discrete model as one unit of evolutionary (coalescent) time in the limit, where $c_N$ is the probability that two individuals picked in a generation have the same parent one generation before. In the discrete models, the population size $N$ is fixed across all generations.\\
Only populations in an equilibrium state are described well by models with fixed population sizes. This idealized condition often does not apply to natural populations. In particular, due to fluctuating environmental conditions population sizes are expected to fluctuate likewise. Two standard models of population size changes are timespans of exponential growth or decline, as well as population bottlenecks, where population size drops to a fixed size smaller than $N$ for a timespan on the evolutionary (coalescent) timescale. Such changes are featured in coalescent simulators as \texttt{ms} \citep{Hudson2002} or \texttt{msprime} \citep{msprime}. The latter changes are also the model of population size changes in \texttt{PSMC} \citep{li2011inference} or similar approaches as \texttt{SMC++} \citep{terhorst2017robust}.  For the Wright-Fisher model, which converges to Kingman's $n$-coalescent if population size $N$ is fixed for all generations, the same scaling $c_N^{-1}$ from discrete genealogy to limit is valid for population size changes which are not extreme (of order $N$ on the coalescent time scale), see \cite{griffiths1994sampling} or \cite{Kaj2003}. The resulting limit process is Kingman's $n$-coalescent, whose timescale is (non-linearly) transformed. However, size changes too extreme can yield a non-bifurcating (multiple merger) genealogy, see \citet[Sect. 6.1]{Birkner2009}.\\ 
For $\Lambda$-$n$-coalescents, the link between fluctuating population sizes in the discrete models and the time-change in the coalescent limit is somewhat less established. While conditions for convergence of the discrete genealogies to a limit process are given in \cite{mohle2002coalescent}, no explicit construction of haploid Cannings models leading to an analogous limit, a $\Lambda$-$n$-coalescent with changed time scale, is given. For a specific case, the Dirac $n$-coalescent for an exponentially growing population, such a construction has been given in \cite{Matuszewski2017}, based on the fixed-$N$ Cannings model (modified Moran model) from \cite{Eldon2006}. However, also other $\Lambda$-$n$-coalescents (or Cannings models which should converge to these) with changed time scale have been recently discussed and applied as models of genealogies, see \cite{Spence1549}, \cite{Kato171060} and \cite{alter2016population}. This leads to the goal of this article, which is to extend the approach in \cite{Matuszewski2017} to explicitly give a construction of time-changed $\Lambda$-coalescents as limits of Cannings models with fluctuating population sizes. %Here, such constructions will be provided for simple $\Lambda$-$n$-coalescents and all Beta-$n$-coalescents, whose population sizes are allowed to fluctuate moderately. 
The Cannings models used are modified Moran models, see e.g. \cite{huillet2013extended}, and the Cannings models introduced in \cite{Schweinsberg2003}. The main tool to establish the convergence to the time-changed $\Lambda$-$n$-coalescent is \citet[Thm. 2.2]{mohle2002coalescent}.\\
For diploid Cannings models, the umbrella model  from \cite{koskela2018robust} gives a general framework to add population size changes, selection, recombination and population structure to the fixed-$N$-model. There, if one only considers population size changes, the limit is a time-changed $\Xi$-$n$-coalescent, a coalescent process with simultaneous multiple mergers. The focus in the present paper is slightly different though, the aim is to explicitly construct Cannings models that converge, after linear time scaling, to a time-changed $\Lambda$-$n$-coalescent, while \cite{koskela2018robust} concentrates on the convergence itself.            

\section{Converging to a time-changed coalescent - sufficient conditions}\label{sec:suffcond}
Cannings models \citep{cannings1974latent,Cannings1975} describe the probabilistic structure of the pedigree (offspring-parent relations) of a finite population in generations $v\in\mathbb{Z}=\{\ldots,2,-1,0,1,2\ldots\}$ with integer-valued population sizes $(N_v)_{v\in\mathbb{Z}}$. The $N_v$ individuals in generation $v$ produce $(\nu^{(v)}_1,\ldots,\nu^{(v)}_{N_v})$ offspring, where $\sum_{i=1}^{N_v}\nu^{(v)}_i=N_{v+1}$ and offspring sizes are exchangeable, i.e. $(\nu^{(v)}_1,\ldots,\nu^{(v)}_{N_v})\stackrel{d}{=}(\nu^{(v)}_{\sigma(1)},\ldots,\nu^{(v)}_{\sigma(N_v)})$ for any permutation $\sigma\in S_{N_v}$. The offspring generation $v+1$ then consists of these individuals in arbitrary order (independent of the parents). The case $N_v=N$ for all $v$ is denoted as the fixed-$N$ case.\\From now on, look at the geneology of the population in generation 0. For convenience, denote the generations in reverse order by $r=-v$, i.e. if one looks $i$ generations back, this is denoted by $r=i$. The population sizes $N_r$ are defined relative to a reference size $N$, in a way that if $N\to\infty$, also $N_r\to\infty$. From now on, use $N=N_0$. The goal is to establish a limit process of the discrete genealogies for $N\to\infty$. The discrete genealogy of a sample of size $n$ in generation 0 is a random process $(\mathcal{R}^{(N)}_r)_{r\in\mathbb{N}_0}$ with values in the partitions of $\{1,\ldots,n\}$, where $i,j$ are in the same block of $\mathcal{R}^{(N)}_r$ iff they share the same ancestor in generation $r$.\\ 
The terminology from \cite{mohle2002coalescent} is used with slight adaptations. Let $c_{N,r}$ be the probability that two arbitrary individuals in generation $r-1$ have the same ancestor in generation $r$ in the model with reference population size $N$.  
Define $F_{N}(s)=\sum_{r=1}^{\left[s\right]}c_{N,r}$ and let $G^{-1}_{N}(t)=\inf\left\lbrace s>0: F_N(s)>t\right\rbrace -1$ be its shifted pseudo-inverse. For $l$ and $a_1,\ldots,a_l\geq 1$, set $\Phi^{(N)}_l(r;a_1,\ldots,a_l)$ as the probability that in Generation $r-1$, from $\sum_{i=1}^l a_i$ individuals sampled from in the Cannings model, specific sets of $a_1\geq\cdots\geq a_l$ individuals each find a common ancestor one generation before (generation r), where ancestors of different sets are different.\\  First, recall this special case of \citet[Thm. 2.2]{mohle2002coalescent} 

\begin{corollary}\label{cor:moe2.2easy}
If we satisfy, for any fixed t, 

\begin{align}
&\lim_{N\to\infty} \inf_{1\leq r\leq G^{-1}_{N}(t)} N_r =\infty,\ \ \lim_{N\to\infty} \sup_{1\leq r\leq G^{-1}_{N}(t)} c_{N,r}=0,\label{eq:moe02conds}\\
& \lim_{N\to\infty} \sum_{r=1}^{\mathcal{G}^{-1}_{N}(t)} \Phi^{(N)}_l(r;a_1,\ldots,a_l)=q_{a_1,\ldots,a_l}t<\infty, a_1\geq\ldots\geq a_l\geq 2 \label{eq:moe02conds2}
\end{align}  
the discrete-time coalescent $(\mathcal{R}^{(N)}_{G_N^{-1}(t)})_{t\geq 0}$, so rescaled in time, converges in distribution (Skorohod-sense) to a continuous-time Markov chain with transition function $\exp^{Qt}$. 
\end{corollary}
\begin{remark}
When compared to the original formulation of \citet[Thm 2.2]{mohle2002coalescent}, the limit here can be described as a homogeneous Markov chain with rate matrix $Q$ instead of the more complicated original description of the transition probabilities as a product integral of matrix-valued measures. This directly follows from the stronger condition \eqref{eq:moe02conds2}, where for \citet[Thm 2.2]{mohle2002coalescent} to hold only convergence and not linear dependence on $t$ is needed. Indeed, if \eqref{eq:moe02conds2} holds, the value $\Pi((0,t])$ of the product measure $\Pi$ in \citet[Thm. 2.2]{mohle2002coalescent} has the form $Qt$, where the diagonal entries are the negative of the other entries in the line (it constitutes a generator of the Markov chain). This is stated on \citet[p. 209]{mohle2002coalescent}, see also Eq. (24) therein. Then, the form of the transition function is described on \citet[p. 203]{mohle2002coalescent}.
\end{remark}
Consider a series of fixed-$N$ Cannings models for each $N\to\infty$ with $c_N\to 0$ for $N\to\infty$ and transition probabilities $\Phi^{(N)}_l(a_1,\ldots,a_l)$ for a merger of $a_1,\ldots,a_l\geq 2$ individuals , converging to a $\Lambda$-$n$-coalescent with infinitesimal rates $\phi_l(a_1,\ldots,a_l):=\lambda_{a_1,a_1}1_{\{l=1\}}$ when scaled by $c_N^{-1}$. 
We will establish a  variant of \citet[Corollary 2.4]{mohle2002coalescent}. 
Fix $t>0$. We assume for all $0\leq r \leq \lceil c_{N}^{-1}t\rceil$:
\begin{flushleft}
\begin{itemize}
\item Arbitrary population size changes of order $N$, i.e.
\begin{equation}\label{eq:cond_popsize}
0<N^{-}(t):=c_1(t)N\leq N_r\leq c_2(t)N=:N^{+}(t)<\infty, 
\end{equation} 
for positive and finite functions $c_1,c_2$ on $\mathbb{R}$
 \item
\begin{equation}\label{eq:cond_phi}
\Phi^{(N)}_l(r;a_1,\ldots,a_l)=\Phi^{(N_r)}_l(a_1,\ldots,a_l)+o_{\sum}(c_{N_r})
\end{equation}
\item Controlling the speed of convergence of $c_N$: There exists $M_1(t)$ and $M_2(t)$ with
\begin{equation}\label{eq:cond_speed_cN}
M_1(t)\leq \frac{c_{N_r}}{c_N}\leq M_2(t)
\end{equation}
\end{itemize}
\end{flushleft}

Here, a series of terms is $o_{\sum}(c_N)$ if summing $O(c^{-1}_N)$ of them vanishes, e.g. if these summands divided by $c_N$ have the same null sequence majorant. If Condition \eqref{eq:cond_speed_cN} holds, \eqref{eq:cond_phi} can be equivalently formulated with $c_N$ instead of $c_{N_r}$. Additionally, note that if we choose $l=1$ in Eq. \ref{eq:cond_phi}, we have
\begin{equation}\label{eq:cond_cnr}
M_1(t)c_{N} + o_{\sum}(c_N) \leq c_{N,r} \leq M_2(t)c_{N} + o_{\sum}(c_N)
\end{equation}
for $N\to\infty$. Finally, if \eqref{eq:cond_popsize} is satisfied, Condition \eqref{eq:cond_speed_cN} is also satisfied if $c_N=f(N)$, where $f$ is regularly varying (at $\infty$).
\begin{lemma}\label{lem:cannpopsizetolambda}
Consider a series of Cannings models with reference size $N$ which fulfill conditions \eqref{eq:cond_popsize},\eqref{eq:cond_phi}, \eqref{eq:cond_speed_cN}, $\lim_{N\to\infty}c_N = 0$ and whose genealogies, of a sample of size $n$, are in the domain of attraction of a $\Lambda$-$n$-coalescent $(\Pi_t)_{t\geq 0}$ (rescaled by $c_N^{-1}$). Then, Corollary \ref{cor:moe2.2easy} can be applied, so $(\mathcal{R}_{G_N^{-1}(t)})_{t\geq 0}\stackrel{d}{\to}(\Pi_t)_{t\geq 0}$ in the Skorohod-sense. 
\end{lemma}
\begin{proof}
Size changes of order $N$ satisfy Condition \eqref{eq:moe02conds}, Condition \eqref{eq:moe02conds2} is then satisfied by \eqref{eq:cond_cnr}, which in turn is satisfied due to \eqref{eq:cond_phi} and \eqref{eq:cond_speed_cN}. Also due to \eqref{eq:cond_cnr}, $F_N$ is bounded by 

\begin{equation}\label{eq:generalFNbounds}
[s]M_1(t')c_N+[s]o(c_N)\leq F_{N}(s)\leq [s]M_2(t')c_N+[s]o(c_N)
\end{equation} 
for $N\to\infty$ and $[s]\leq c_{N}^{-1}t'$ and thus its pseudo-inverse by 

$$\frac{t}{M_2(t')c_N}+\frac{o(c_N)}{c_N}-1 \leq \mathcal{G}_N^{-1}(t)\leq \frac{t}{M_1(t')c_N}+\frac{o(c_N)}{c_N}-1$$ with an appropriate $t'\geq t$. This implies that the time change function $\mathcal{G}_N^{-1}$ for the discrete models in Corollary \ref{cor:moe2.2easy} is of order $c^{-1}_N$. Knowing this, we compute 

\begin{align*}
\lim_{N\to\infty} \sum_{r=1}^{\mathcal{G}^{-1}_{N}(t)} \Phi^{(N)}_l(r;a_1,\ldots,a_l)\stackrel{\eqref{eq:cond_phi}}{=}&\lim_{N\to\infty} \sum_{r=1}^{\mathcal{G}^{-1}_{N}(t)}\underbrace{\Phi^{(N_r)}_l(a_1,\ldots,a_l)c_{N_r}^{-1}}_{\to \phi_l(a_1,\ldots,a_l)}c_{N_r}\\ \stackrel{\eqref{eq:cond_phi}}{=}&\phi_l(a_1,\ldots,a_l)\left(\underbrace{\sum_{r=1}^{\mathcal{G}^{-1}_{N}(t)}c_{N,r}}_{=F_N(\mathcal{G}^{-1}_{N}(t))}+ \underbrace{\sum_{r=1}^{\mathcal{G}^{-1}_{N}(t)} o_{\sum}(c_N)}_{\to 0} \right) \\=&\phi_l(a_1,\ldots,a_l)t.
\end{align*}

The second equation is valid due to the uniform convergence of\\ $\Phi^{(N_r)}_l(a_1,\ldots,a_l)c_{N_r}^{-1}$ in $r$ for $N\to\infty $ ($N_r$ is bounded from below on the timescale used). This allows to pull out $\phi_l(a_1,\ldots,a_l)$. This establishes the convergence of     
$(\mathcal{R}_{G_N^{-1}(t)})_{t\geq 0}$ to the same $\Lambda$-$n$-coalescent as the fixed-size model. 
\end{proof}
\begin{remark}\label{rem:lintsc} If $\mathcal{G}^{-1}(t):=\lim_{N\to\infty} \mathcal{G}_N^{-1}(t)c_N$ exists, we have, with $\mathcal{G}=(\mathcal{G}^{-1})^{-1}$,
\begin{equation}\label{eq:lineartimescale_limitcoal}
(\mathcal{R}^{(N)}_{[t/c_N]})_{t\geq 0}\stackrel{d}{\to} (\Pi_{\mathcal{G}(t)})_{t\geq 0}
\end{equation}  
for $N\to\infty$, as described in \citet[Sec. 4]{moehle_robust1998}. This is a weak condition, since $G_N^{-1}(t)$ is of order $c^{-1}_N$.\\ Let mutation be introduced in the discrete model by allowing mutations from parent to offspring with a rate $\mu_N$. Consider $\mu_Nc_N^{-1}\to \theta$. If we now scale as in Eq. \eqref{eq:lineartimescale_limitcoal}, the mutations on the time-scaled $\Lambda$-$n$-coalescent are given by a Poisson point process with homogeneous intensity $\theta$. 
\end{remark}

%If we have even $c^{-1}_Nc_{N,r}=f(r)+o(f(N))$, we can see $F_N(c_N^{-1}t)=\sum^{[c_N^{-1}t]}_{r=1} f(r)c_N$ as a Riemann sum and we have $\lim_$  
\section{Modified Moran models with fluctuating population size}\label{sec:3M}
In the fixed-$N$ setting, models leading to a multiple merger $\Lambda$-$n$-coalescent feature skewed offspring distributions. The simplest such example are models where only a single individual even has more than one offspring (and occasionally has many offspring), the modified Moran models. Following \cite{huillet2013extended}, define the modified (haploid) Moran model with fixed population size $N$. Let $(U_N(z))_{z\in\mathbb{N}}$ be i.i.d. random variables with values in $\{2,\ldots,N\}$, let $U_N$ be a r.v. with their common distribution. In each generation $z\in\mathbb{Z}$,
\begin{itemize}
\item One randomly chosen individual has $U_N(z)$ offspring,
\item $U_N(z)-1$ randomly chosen individuals have no offspring,
\item The other $N-U_N(z)$ have one offspring each,
\end{itemize} 
which defines a Cannings model with population size $N$.\\
The focus will be on such models with $U_N/N\stackrel{d}{\to}0$ for $N\to\infty$, which is equivalent to $c_N\to 0$ \citet[Lemma 3.2]{huillet2013extended}.
%We further assume $c_N\sim c N^{-a}$ for $N\to\infty$ with $a\geq 1$, where $c_N$ is the coalescence probability, i.e. the probability that 2 randomly chosen individuals have a common parent, and $c>0$ a constant. 
We further assume, for each $k\geq 2$,
\begin{equation}\label{eq:modmoran_Lambda}
\lim_{N\to\infty}\frac{E((U_N)_k)}{N^ {k-2}E((U_N)_2)}=\lim_{N\to\infty}\frac{E((U_N)_k)}{(N)_kc_N}=:\phi_k
\end{equation}
exists, where $(x)_k:=x(x-1)\cdots(x-k+1)$ is the falling factorial. Then, \citet[Thm 3.3]{huillet2013extended} ensures that the genealogy of a sample of size $n$ in the modified Moran model converges to a $\Lambda$-$n$-coalescent, if we rescale time by dividing by $c_N=\frac{E((U_N)_2)}{(N)_2}$, and that $(\phi_k)_{k\geq 2}$ uniquely defines $\Lambda$, i.e. $\phi_k=\int x^{k-2} \Lambda(dx)=\lambda_{k,k}$ ($\Lambda$ is a finite measure on a compact set and thus uniquely defined by its moments).\\  
To use the general approach from \cite{mohle2002coalescent} as outlined in the previous section for modified Moran models, one first needs to explain how the population size changes from generation to generation and how the relationship between offspring and parent generation is defined. If population size declines from generation $r$ to $r-1$, e.g. sample $N_{r-1}$ individuals randomly (without replacement) from $N_{r}$ potential offspring consisting of $U_{N_r}$ offspring of the multiplying parent and $N_{r}-U_{N_r}$ single offspring. In other words, the model produces potential offspring as in the fixed-$N_r$ model and then samples the next generation from these. The next proposition shows that such downsampling, for  modified Moran models, leads to genealogies converging to a time-changed $\Lambda$-$n$-coalescent.\\
If individuals are added to the population (population growth), i.e. 
\begin{equation}\label{eq:def_popsizechange}
d_{N,r}=N_{r-1}-N_r,
\end{equation} many individuals, 
one could simply add them as further offspring of the already multiplying parent (which now has $U_{N,r}\stackrel{d}{=}U_N+d_{N,r}$ offspring), as in \citep{Matuszewski2017}.  This allocation scheme will be called 'single expansion' $(\mathcal{SE})$.
\begin{remark}
Depending on the magnitude of population size increase, this can strongly increase coalescence probabilities. For instance, for a population expansion of size $Nm$, if one just expands by adding $d_{N,r}=Nm$ to the offspring number of the individual with multiple offspring in a single generation, the coalescence probability for this generation is dominated by the population size change. Then $U_{N,r}\geq Nm$, leading to $c_{N,r}=\frac{E((U_{N,r})_2)}{(N_{r-1})_2}\geq \frac{(Nm-1)^2}{(N_{r-1})_2}=O(1)\nrightarrow 0$ for $N\to\infty$. Thus, from generation $r-1$ to $r$, coalescence is still happening with positive probability for $N\to\infty$, which shows that a potential limit coalescent cannot just be a (non-degenerately) time-changed $\Lambda$-$n$-coalescent, a continuous-time (inhomogeneous) Markovian process. This has an implication for modelling of real populations: The genealogy of a sudden population expansion, happening at a specific generation, where a single genotype/individual is responsibly for the population growth, is not given by a time-changed continuous-time $\Lambda$-$n$-coalescent.
\end{remark}
 
%A second option is letting individuals added pick their parents randomly, as in the Wright-Fisher model. Clearly, the resulting model is not a modified Moran Model anymore, since multiple mergers can happen in a single generation. Thus, individuals can either coalesce when sharing the multiplying individual as a parent or when having any other as parent. A binomially distributed number $D_{N,r}\stackrel{d}{=}Bin(d_{N,r},N_r^{-1})$ of added individuals will choose the already multiplying parent. The probability $\kappa_{N,r}$ that there is any merger of $a$ individuals sampled in generation $r-1$ having a different parent than the multiplying parent thus satisfies
%\begin{equation}\label{eq:WFMcomponent}
%\kappa_{N,r}\leq 1-\left(\frac{N_r}{N_r+d_{N,r}}\right)^{a}\leq 1-\left(1-\frac{d_{N,r}}{N_r}\right)^{a},
%\end{equation} 
%which is of order $O(N^{-1}d_{N,r})$ \fab{This is shown in the supercritical branching part, move this proof either here or to the appendix...}. If this is also $o_{\sum}(c_N)$, we can ignore such coalescences when applying \ref{lem:cannpopsizetolambda}. We denote this allocation scheme with $(\mathcal{WF})$.\\ 
A second option is to only add at most $U_{N_r}-1$ individuals as  offspring of the non-reproducing individuals in the fixed-$N$ approach, which means at least one individual can be added. However, if $Nc_N\to 0$, this allows even instantaneous population expansions of order $N$ by adding one individual for $O(N)$ generations. This allocation scheme is called 'relaxed Moran' $(\mathcal{RM})$.\\
The following proposition provides criteria for genealogies in these modified Moran models with fluctuating population sizes so that they converge to a time-changed $\Lambda$-$n$-coalescent. 
\begin{proposition}\label{lem:3Mconv}
Consider a fixed-$N$ modified Moran model and $(N_r)_{r\in\N}$ so that $U_N/N\stackrel{d}{\to} 0$ for $N\to\infty$, satisfying also Eq. \eqref{eq:cond_popsize}, \eqref{eq:cond_speed_cN} and \eqref{eq:modmoran_Lambda}. If $d_{N,r}>0$, set $s_{N,r}=\frac{d_{N,r}}{N}$ and assume $s_{N,r}\leq d_N\to 0$. Add individuals with the following allocation schemes and additional constraints 
\begin{itemize}
\item Under $\mathcal{(SE)}$, assume $\frac{E(U_N)}{E((U_N)_2)}\to 0$ and
$s_{N,r}\leq c_4N^{-1}E(U_N)$ for $r\leq c^{-1}_Nt$, a constant $c_4>0$ and $N\to\infty$.
%\item Under $\mathcal{(WF)}$, assume $s_{N,r}\leq d_N=o(c_N)$ and $(Nc_N)_{N\in\mathbb{N}}$ bounded.
\item Under $\mathcal{(RM)}$, assume $d_{N,r}\leq \min\{i:P(U_{N_r}=i)>0\}$ %and $Nc_N\to 0$ for $N\to\infty$
\end{itemize} 
Based on the fixed-size modified Moran model and $(N_r)_{r\in\N}$  define a modified Moran model with population sizes $(N_r)_{r\in\N}$ and offspring variable $U_{N,r}$ following the chosen allocation scheme.\\ 
Then, 
 $(\mathcal{R}_{G_N^{-1}(t)})_{t\geq 0}\stackrel{d}{\to}(\Pi_t)_{t\geq 0}$ in the Skorohod-sense, where $(\Pi_t)_{t\geq 0}$ is the coalescent limit for the fixed-$N$ modified Moran model. 
\end{proposition}

\begin{proof}
This is shown by applying Lemma \ref{lem:cannpopsizetolambda}. All conditions but \eqref{eq:cond_phi} of it are fulfilled under the assumptions of the proposition currently proved ($U_N/N\to 0\Leftrightarrow c_N\to 0$). Thus, we only need to show that \eqref{eq:cond_phi} is satisfied.\\
From \citet[Sect. 2]{huillet2013extended}, recall that for a fixed-$N$ modified Moran model $c_N=E((U_N)_2)/(N)_2$ and $\Phi^{(N)}_l(a_1,\ldots,a_l)=1_{\{l=1\}}\frac{E((U)_{a_1})}{(N)_{a_1}}$.\\ 
First, assume $d_{N,r}\geq 0$. Let $A_{n,r}$ be the additional offspring added to the multiplying parent. Then, %A independent of U

\begin{align}\label{eq:fact_osumcn}
&\frac{E((U_{N_r}+A_{N,r})_{a_1})}{(N_r)_{a_1}c_N}=\sum_{k=1}^{a_1}s(a_1,k)\sum_{l=0}^k\binom{k}{l}\frac{E(U_{N_r}^l)A_{N,r}^{k-l}}{(N_r)_{a_1}c_N}\nonumber\\=&\frac{E((U_{N_r})_{a_1})}{(N_r)_{a_1}c_N}+\sum_{k=1}^{a_1}s(a_1,k)\underbrace{\sum_{l=0}^{k-1}\binom{k}{l}\frac{E(U_{N_r}^l)A_{N,r}^{k-l}}{(N_r)_{a_1}c_N}}_{\to 0}
\stackrel{\eqref{eq:modmoran_Lambda}}{\to} \phi_k 
\end{align}
%version for random A
%\begin{align}\label{eq:fact_osumcn}
%&\frac{E((U_{N_r}+A_{N,r})_{a_1})}{(N_r)_{a_1}c_N}=\sum_{k=1}^{a_1}s(a_1,k)\sum_{l=0}^k\binom{k}{l}\frac{E(U_{N_r}^l)E(A_{N,r}^{k-l})}{(N_r)_{a_1}c_N}\nonumber\\=&\frac{E((U_{N_r})_{a_1})}{(N_r)_{a_1}c_N}+\sum_{k=1}^{a_1}s(a_1,k)\underbrace{\sum_{l=0}^{k-1}\binom{k}{l}\frac{E(U_{N_r}^l)E(A_{N,r}^{k-l})}{(N_r)_{a_1}c_N}}_{\to 0}
%\stackrel{\eqref{eq:modmoran_Lambda}}{\to} \phi_k 
%\end{align}
uniformly in $r$ (convergence is at least as fast as for $N^-(t)$),
 where $s(n,k)$ are Stirling numbers of the first kind. Under allocation scheme $(\mathcal{RM})$, $A_{N,r}=0$ and thus the second sum equals 0. %For $l=0$, the inner summand in \eqref{eq:fact_osumcn} vanishes uniformly in in $0\leq r \leq c_{N}^{-1}t$ since,  
%$$\frac{d_{N,r}^{k}}{(N_r)_{a_1}c_N}=\frac{s_{N,r}^{k}}{N_r^{a_1-k}c_N}\frac{N_r^{a_1}}{(N_r)_{a_1}}\stackrel{a_1\geq 2}{\leq} \frac{c_4E(U_N)}{E(U_N(U_N-1))}\frac{a_1^{a_1}NN^+(t)}{a_1!(N)_2}\to 0,$$
%where we can omit powers of $s_{N,r}\leq 1$ for large $N$.

To see that the inner sum in \eqref{eq:fact_osumcn} also vanishes for the allocation scheme $(\mathcal{SE})$, first observe that 
\begin{equation}\label{eq:supa_addindeffect}
\frac{E(U_{N_r}^l)E(A_{N,r}^{k-l})}{(N_r)_{a_1}c_N}\leq \frac{E((N_r^{-1}A_{N,r})^{k-l})N_r^{a_1}}{N_r^{a_1-l-(k-l)}c_N(N_r)_{a_1}} \leq \frac{E((N_r^{-1}A_{N,r})^{k-l})a_1^{a_1}}{N_rc_Na_1!},
\end{equation}
where we can omit factors $U_{N_r}/N_r\leq 1$. The inequality $\frac{N_r^{a_1}}{(N_r)_{a_1}}\leq \frac{a_1^{a_1}}{a_1!}$ follows from the fact that $x\mapsto\frac{x^{a_1}}{(x)_{a_1}}$ decreases for $x\geq a_1$.\\
%For $(\mathcal{WF})$, recall $A_{N,r}$ is $Bin(d_{N,r},N_r^{-1})$ distributed and independent of $U_{N_r}$. Thus, $A_{N,r}N_r^{-1}\in[0,1]$ and $E((N_r^{-1}A_{N,r})^{k-l})\leq E(N_r^{-1}A_{N,r})=(N_r)^{-2}d_{N,r}\leq s_{N,r}\leq d_N\to 0$ and $N_rc_N$ bounded. This shows that Eq. \eqref{eq:supa_addindeffect} converges to 0 for this scheme (uniformly in $r$). 
For $(\mathcal{SE})$, $A_{n,r}=d_{N,r}$ and thus for $0\leq r \leq c_{N}^{-1}t$ and $0\leq l< k<a_1$,

\begin{align*}
\eqref{eq:supa_addindeffect}\leq& \frac{E((c_4N^{-1}U_N)^{k-l})a_1^{a_1}}{N_rc_Na_1!}\leq\frac{c_4^{k-l}E(U_N)a_1^{a_1}}{NN^-(t)c_Na_1!}=\frac{E(U_N)(N)_2a_1^{a_1}c_4^{k-l}}{E((U_N)_2)NN^-(t)a_1!}\to 0
\end{align*} 
for $N\to\infty$.\\
Both allocation schemes $(\mathcal{SE})$ and $(\mathcal{RM})$ still result in modified Moran models with a single multiplying parent, so to show Eq. \eqref{eq:cond_phi} one only needs to show $\Phi_1^{(N)}(r;a_1)=\Phi_1^{(N_r)}(a_1)+o_{\sum}(c_N)$ for $0\leq r \leq c_{N}^{-1}t$. %However, for $(\mathcal{WF})$, the probability $\kappa_{N,r}$ of having any merger with an other parent than the multiplying parent, Eq. \eqref{eq:WFMcomponent} is $O(N_r^{-1}d_{N,r})$, so with $N_r^{-1}d_{N,r}\leq d_N=o(c_N)$,  $\kappa_{N,r}$ is $o_{\sum}(c_N)$. Thus, $\Phi_1^{(N)}(r;a_1,\ldots,a_l)=0+o_{\sum}(c_N)=\Phi_1^{(N_r)}(a_1,\ldots,a_l)$ if $l\geq 2$. 
Following \citet[Eq. (2)]{mohle2002coalescent} applied for the modified Moran model with $U_{N,r}$ distributed as $U_{N_r}+d_{N,r}$,

\begin{align*}
&\Phi^{(N)}_l(r;a_1)=E((U_{N_r}+d_{N,r})_{a_1})/(N_r+d_{N,r})_{a_1}\\
=&  \frac{(N_r)_{a_1}}{(N_r+d_{N,r})_{a_1}}E((U_{N_r}+d_{N,r})_{a_1})/(N_r)_{a_1}\\ \stackrel{(*)}{=}&(1-o(1))^{-1}\left(\frac{E((U_{N_r})_{a_1})}{(N_r)_{a_1}}+o_{\sum}(c_N)\right)=\Phi^{(N_r)}_1(a_1)+o_{\sum}(c_N).
\end{align*}
Equation $(*)$ follows from \eqref{eq:fact_osumcn} and, for the first factor, from $s_{N,r}\leq d_N$ being a null sequence for any allocation scheme.\\
Now, consider $d_{N,r}<0$. Then, we get the offspring population by sampling $N_{r-1}$ individuals out of $N_r$, from which $U_{N_r}$ share one common parent. Thus, this is again a modified Moran model, where  
$U_{n,r}$ is conditionally hypergeometrically distributed with $P(U_{N,r}=k|U_{N_r})=\frac{\binom{U_{N_r}}{k}\binom{N_r-U_{N_r}}{N_{r-1}-k}}{\binom{N_r}{N_{r-1}}}$. 
Using the factorial moment of the hypergeometric distribution leads to


\begin{align*}
& \Phi^{(N)}_1(r;a_1)= E\left(\frac{(U_{n,r})_{a_1}}{(N_{r-1})_{a_1}}\right)=\frac{E((U_{n,r})_{a_1}\vert U_{N_r})}{(N_{r-1})_{a_1}}=\frac{(N_{r-1})_{a_1}}{(N_{r-1})_{a_1}}\frac{E((U_{N_r})_{a_1})}{(N_r)_{a_1}}
\\=&\Phi^{(N_r)}(a_1),
\end{align*} 
\end{proof}

\begin{remark}\label{rem:moranincluded}
%The conditions of Lemma \ref{lem:3Mconv} are just sufficient and not necessary. However, a rather tight control of $c_N$ is needed since we want to scale linearly by $c_N$ to impose a simple Poissonian mutation model (Remark \ref{rem:lintsc}). This forces conditions like \eqref{eq:cond_phi}. Additionally, to explicitly define the discrete model as a modified Moran model needs some control of how the population size is changed and how this affects the offspring number of the individual who has more than one offspring. 
For allocation scheme $(\mathcal{RM})$, the classic Moran model converging to Kingman's $n$-coalescent fulfills the conditions of the proposition above.
\end{remark}
For any $\Lambda$-$n$-coalescent with $\Lambda([0,1])=1$, \citet[Prop. 3.4]{huillet2013extended} shows that there always exist fixed-$N$ modified Moran models such that there rescaled genealogies converge to the $\Lambda$-$n$-coalescent. These can be constructed via a random variable $U'_N$, that is distributed like the merger size of the first merger in a $\Lambda$-$N$-coalescent. As shown in \citep[Eq. 9]{huillet2013extended}, this means
\begin{equation}\label{eq:LambdamodMoran}
P(U'_N=j)=\lambda_N^{-1} \binom{N}{j}E(X^{J-2}(1-X)^{N-j}), j\geq 2,
\end{equation}
where $\lambda_N$ is the total rate of the $\Lambda$-$N$-coalescent and $X$ has distribution $\Lambda$. 
Eq. \eqref{eq:LambdamodMoran} further implies
\begin{equation}\label{eq:3M_factmom}
E((U'_N)_k)=\frac{(N)_k}{\lambda_N}E(X^{k-2})
\end{equation}
for all $k\geq 2$, see \citet[Eq. 10]{huillet2013extended}, and \citet[Remark p.9]{huillet2013extended} shows  
\begin{equation}\label{eq:EUN_3M}
E(U'_{N})=\frac{(N)_2}{\lambda_N}P(X=0)+\frac{N}{\lambda_N}\left(E\left(\frac{1-(1-X)^{N-1}}{X}1_{\{X\in(0,1)\}}\right)+P(X=1)\right).
\end{equation}
\\ 
If $\int x^{-2}\Lambda(dx)=\infty$, setting $U_N=U'_N$ leads to $c_N\to 0$ ($\Leftrightarrow N^{-1}U_N\stackrel{d}{\to} 0$) and satisfies Condition \eqref{eq:modmoran_Lambda}. Thus, the genealogy of $n$ individuals (rescaled by $c_N^{-1}$) in the fixed-$N$ model converges to the $\Lambda$-$n$-coalescent, see \citet[Prop. 3.4]{huillet2013extended}. To show that there is convergence also for genealogies with variable population sizes of order $N$, i.e. \eqref{eq:cond_popsize} is satisfied, Proposition \ref{lem:3Mconv} applies if additionally Condition \eqref{eq:cond_speed_cN} and, if there is population growth in any generation, further conditions based on the allocation scheme holds.\\ At least for $\Lambda=\beta(a,b)$ for $a\in(0,2]$, \eqref{eq:cond_speed_cN} is satisfied. \citet[Eq. (10)+Corallary A.1]{huillet2013extended} shows that for $a<2$ one has $c_N\sim \frac{(2-a)\Gamma(b)}{\Gamma(a+b)}N^{a-2}$, while for $a=2$, this is $c_N\sim (b(b+1)\log_N)^{-1}$. Both are regularly varying, thus satisfy \eqref{eq:cond_speed_cN}.\\  
Now, switch to the case $\int x^{-2}\Lambda(dx)<\infty$. Then, $\lambda_N\to\lambda<\infty$ for $N\to\infty$. Consider a slight variant of the construction of $U_N$ in the proof of \citet[Prop. 4]{huillet2013extended}, to end up with a modified Moran model where there is always one individual with multiple offspring, see also \citet[Example 4.1]{huillet2013extended}: Define $U_N=U'N1_{A_N}+2(1-1_{A_N})$ for sets $A_N$ s.t. $U'N$,$1_{A_N}$ are independent and $P(A_N)=N^{-\gamma}$ for $1<\gamma<2$. Let $c'_N=E((U'_N)_2)/((N)_2)=\lambda_N^{-1}\to \lambda>0$ for $N\to\infty$. Then, for $k>2$,

\begin{align}\label{eq:thin3M}
&c_N=((N)_2)^{-1}E((U_N)_2)\stackrel{\eqref{eq:3M_factmom}}{=}\lambda_N^{-1}N^{-\gamma}+(1-N^{-\gamma})\frac{2}{N(N-1)}\to 0,
\\&
\frac{E((U_N)_k)}{(N)_k c_N}=\frac{E(X^{k-2})N^{-\gamma}}{\lambda_N c_N }=\frac{E(X^{k-2})N^{-\gamma}}{\lambda_N\lambda_N^{-1}N^{-\gamma}}\frac{\lambda_N \lambda_N^{-1}N^{-\gamma}}{\lambda_N^{-1}N^{-\gamma}+(1-N^{-\gamma})\frac{2}{N(N-1)}}\nonumber \\ & \to E(X^{k-2})\nonumber%\\
%&\frac{E(U_N)}{E((U_N)_2)}
\end{align} 
since, on the complement of $A_N$, $(U'_N)_k=\delta_{k,2}$ for $k\geq 2$. The second equation is equivalent to fulfilling \eqref{eq:modmoran_Lambda}, so there is convergence to the $\Lambda$-$n$-coalescent for the chosen $\Lambda$. Again, $c_N=f(N)$ with $f$ regularly varying, so Eq. \eqref{eq:cond_speed_cN} is fulfilled. Thus, \ref{lem:3Mconv} can be applied if the allocation-scheme specific conditions are also fulfilled.
\begin{remark}\label{rem:diffmodMoran}\ \\
\begin{itemize}
\item There is a biological interpretation of the modified Moran models defined by \eqref{eq:LambdamodMoran} in the fixed-$N$ setting ($U_N=U'_N$). Choose one multiplying individual and one non-reproducing individual at random. Every other individual reproduces once (or survives) with probability $X$, which has distribution $\Lambda$. All "missing" individuals in the next generation get replaced by offspring of the multiplying individual. If instead $U_N=U'N1_{A_N}+2(1-1_{A_N})$ is used, this reproduction pattern only appears occasionally in some generations (with probability $N^{-\gamma}$ per generation). 
\item Interestingly, as also discussed in \cite{huillet2013extended}, very different modified Moran models can lead to the same $\Lambda$-$n$-coalescent limit in the fixed-$N$ setting. For instance, the modified Moran model above for $\Lambda=\delta_p$, $p\in(0,1]$ leads to the Dirac-$n$-coalescent, which is also the limit of a modified Moran model with $U_N=Np1_{A_N}+2(1-1_{A_N})$, see \cite{Eldon2006}. The rare large family has constant size $pN$ in the second model, while in the first model its size is binomially distributed with mean $pN$ and variance $Np(1-p)$ of the same order. This second model was used in \cite{Matuszewski2017} for an exponentially growing population (on the coalescent time scale), which also fulfills the assumptions of Proposition \ref{lem:3Mconv}. A similar class of models can also be found for Beta $n$-coalescents, see e.g. \cite{hartmann2018large}.\\There is also a somewhat similar model as this binomial sampling presented here in \cite{eldon2012age}, where a Poissonian model is used - however, not a fixed-$N$ model. 
\item The condition of $\Lambda([0,1])=1$ is not very important: If one scales by $c_2c_N$ instead of $c_N$ for any $c_2>0$, the rescaled discrete genealogies converge to the $c_2\Lambda$-$n$-coalescent. 
\item The construction as a limit of a modified Moran model when only allowing big values of $U_N$ with probability $N^{-\gamma}$ also works for $\Lambda$-$n$-coalescents with $\int x^{-2}\Lambda(dx)=\infty$. This will be needed later to force $c_N=o(N^{-1})$, if it originally is not. Choose $U_N=U'N1_{A_N}+2(1-1_{A_N})$ instead of just $U_N=U_N'$ and tune $P(A_N)$ so that $c'_NP(A_N)=((N)_2)^{-1}E((U'_N)_2)P(A_N)=N^{-\gamma}$ for $\gamma\in(1,2)$. Then, also Eqs. \eqref{eq:thin3M} are fulfilled and thus the modified Moran models with "thinned" large families converge to the same $\Lambda$-$n$-coalescent and also satisfy Eq. \eqref{eq:cond_speed_cN}. This works for any family of modified Moran models in the fixed-$N$ setting that converge to any $\Lambda$-$n$-coalescent.
\end{itemize}
\end{remark}

This shows that the presented models satisfy the conditions of Proposition \ref{lem:3Mconv} apart from the allocation-model specific ones.  
Which allocation scheme now allow for exponential growth and instantaneous population expansions (if such population expansions are possible, also any other growth of order $N$ is allowed)?\\
First, consider any modified Moran model with $E((U_N)_2)\to\infty$ for $N\to\infty$. Then, as in \citet[third remark p. 8]{huillet2013extended}, one has 

$$\frac{E(U_N)}{E((U_N)_2)}\sim \frac{E(U_N)}{E(U_N^2)}\leq \frac{1}{E(U_N)}.$$ 
This fraction thus converges to 0 regardless of whether $E(U_N)\to \infty$ or not. 
All presented fixed-$N$ modified Moran models with $E((U_N)_2)\to\infty$ fulfill the conditions of Proposition \ref{lem:3Mconv} for the allocation scheme $(\mathcal{SE})$ if at most $d_{N,r}\leq c_4E(U_N)$ individuals are added in a generation. This is $o(N)$, since $N^{-1}U_N\stackrel{d}{\to} 0$ but allows for adding up to any fixed number $k\in\mathbb{N}$ individuals per generation. For exponential growth with constant rate $\rho>0$, i.e. if $N_r=\lceil N(1-c_N\rho)^r \rceil$, one needs ($N_0=N$)

\begin{align*}
d_{N,r} &=\lceil N( 1-c_N\rho)^{r}\rceil -\lceil N( 1-\rho c_N)^{r+1}\rceil
\leq N\left( 1 - \left( 1-\rho c_N\right)\right)+1\\
&= N(\rho c_N)+1
\end{align*}
for any $\epsilon>0$. Again as in Eq. \eqref{eq:EUN_3M}, \citet[Remark p.9]{huillet2013extended} shows $E(U_N)=c_5Nc_N$ for a constant $c_5$, so such growth is covered (if $Nc_N\to 0$, we just need to add at most one individual, which is allowed as described above). For Dirac $n$-coalescents with exponential growth, this was shown in \citep{Matuszewski2017}.\\
If $E((U_N)_2)\nrightarrow \infty$, assume that it is bounded (if instead a subsequence $\to\infty$, we just don't define the discrete model for all generations $N$, we can then define a limit on either a subsequence $\to\infty$ or bounded). Then, $c_N=O(N^{-2})$ and the allocation scheme $(\mathcal{RE})$ allows for any population size change covered by Eq. \eqref{eq:cond_popsize}, since it is enough to add at most a single individual in $O(N)$ generations.\\
This argument shows that any population size change (especially instantaneous population expansions on the coalescent time scale) can be accomodated if $Nc_N\to 0$, i.e. it is enough to add at most a single individual per generation. As shown in Remark \ref{rem:diffmodMoran}, any $\Lambda$-$n$-coalescent can be seen as a limit of modified Moran models with $c_N=N^{-\gamma}$ for $1<\gamma<2$ which fulfill $Nc_N\to 0$. This shows that one can always define modified Moran models with fluctuating population sizes so that they converge to the $\Lambda$-$n$-coalescent with a time change. The question is whether this technical approach of "thinning" the large-offspring events of $U_N$ is justified when modelling a biological population.   
\subsection{Shifting the time change to the limit process}\label{sec:scaletolim}
As described in the last section, for any $\Lambda$-$n$-coalescents there are time-changed versions constructed as time-scaled limits of modified Moran models with varying population sizes that satisfy  $c_N=bN^{-\gamma}+o_{\sum}(c_N)$, $\gamma,b>0$, which is stronger than Condition \eqref{eq:cond_cnr}. For these modified Moran models and any population size changes fulfilling the conditions of Proposition \ref{lem:3Mconv}, this section shows that Remark \ref{rem:lintsc} applies and we can describe the time scaling $\mathcal{G}$ from \eqref{eq:lineartimescale_limitcoal} of the limit coalescent process in more detail for the Beta and simple $n$-coalescents described above. $\mathcal{G}$ is the pseudo-inverse of $\lim_{N\to\infty}\mathcal{G}^{-1}_Nc_N$, so   
\begin{equation}\label{eq:compute_mathcalG}
\mathcal{G}(t)=\lim_{N\to\infty} F_N(tc_{N}^{-1}),
\end{equation}
since for a series of functions, the inverses converges iff the original functions converge and since $cf$  has the inverse $t\mapsto f^{-1}(c^{-1}t)$. %\fab{CITATIONS? CONDITIONS FOR FIRST, CONTINUITY? PROVED FIRST CASE IN MY DIPLOMA THESIS FOR SKOROHOD TOPOLOGY AND A SPECIAL CASE...)} 
It is important to note here that any terms of order $o_{\sum}(c_N)$ can be omitted when computing $F_N$. Thus, we can replace $c_{N,r}$ by $c_{N_r}$ and even by $c^*_{N_r}=c_2N_r^{-\gamma}$ for a constant $c_2$ and $\gamma>0$. Furthermore, assume that $N^{-1}N_{\lfloor tc_N^{-1}\rfloor +1}\to \nu(t)$, analoguous to \cite{griffiths1994sampling}. Then,

\begin{align*}
\mathcal{G}(t)=&\lim_{N\to\infty}\sum_{r=1}^{[tc_{N}^{-1}]} \frac{c^*_{N_r}}{c^*_N}c^*_N=\lim_{N\to\infty} \sum_{r=1}^{[tc_{N}^{-1}]} \left(\frac{N}{N_r}\right)^{\gamma}c^*_N\\=&\lim_{N\to\infty}\int_0^t \sum_{r=1}^{[tc_N^{-1}]} \left(\frac{N_r}{N}\right)^{-\gamma}1_{[(r-1)c_N,rc_N)}(s) \lambda(ds) = \int_0^t (\nu(s))^{-\gamma} ds, 
\end{align*}
where for convergence, observe that there is pointwise convergence 

$$ \sum_{r=1}^{[tc_N^{-1}]} \left(\frac{N_r}{N}\right)^{-\gamma}1_{[(r-1)c_N,rc_N)}(s)= \left(\frac{N_{\lfloor sc_N^{-1}\rfloor+1}}{N}\right)^{-\gamma}\to (v(s))^{-\gamma}$$
for $s\in[0,t]$ inside the integral and that bounded convergence is applicable since the integrand is in $[0,1]$.
\begin{remark}\ 
\begin{itemize}
\item The integral representation of the time change is a deterministic version of the coalescent intensity from \citet[Sect. 1.3]{Kaj2003}, just applied to Cannings models leading to non-Kingman $\Lambda$-$n$-coalescents.
\item  As described in \citet[Section 4]{moehle_robust1998}, the timechanged $\Lambda$-$n$-coalescent limit can also be expressed by its infinitesimal rates 

$$\lambda^{(\nu)}_{n,k}=(\nu(s))^{-\gamma}\int^1_0 x^{k-2}(1-x)^{n-k}\Lambda(dx)$$ for a merger of $k$ of $n$ present lineages. This is also the form in which the limit process of the diploid umbrella model from \cite{koskela2018robust} is given.
\item Conditioned that the limit coalescent $(\Pi_{\mathcal{G}(t)})_{t\geq 0}$ has at time $T_0=t_0$ coalesced into a state with $b$ blocks, what is the distribution of the waiting time $T$ for the next coalescence event? If $T=t$, this means that in the non-rescaled $\Lambda$-$n$-coalescent $(\Pi_t)_{t\geq 0}$, we wait $\mathcal{G}(t)-\mathcal{G}(t_0)$ for the next coalescence. This waiting time $T'$ in $(\Pi_t)_{t\geq 0}$  is exponentially distributed with parameter $\lambda_n$ (total rate of coalescence). Thus, 
\begin{equation}\label{eq:cond_coaldist}
P(T>t_0+t|T_0=t_0)=P(T'>\mathcal{G}(t_0+t)-\mathcal{G}(t_0))=e^{\lambda_b(\mathcal{G}(t_0+t)-\mathcal{G}(t_0))}.
\end{equation}
\end{itemize}
\end{remark}
As a simple application, to model exponential population growth on the coalescent time scale, set $\frac{N_{c_N^{-1}t}}{N}\sim(1-\rho c_N)^{c_N^{-1}t}\to exp(-\rho t)$. In this case, $\mathcal{G}(t)=\int_0^t e^{\rho\gamma s}ds=(\rho\gamma)^{-1}(e^{\rho\gamma t}-1)$. For Dirac coalescents ($\Lambda=\delta_p$) and a modified Moran taking only values $Np$ and 2, this was shown already in \citet[Eq. (41)]{Matuszewski2017} (which also falls in the class of models discussed here, see Remarks \ref{rem:diffmodMoran}).\\
The waiting times for coalescence events in case of exponential growth are Gompertz-distributed, as for Kingman's $n$-coalescent with exponential growth (e.g. see \citet[Eq. 5]{slatkin1991pairwise}, \cite{polanski2003note}). From Eq. \eqref{eq:cond_coaldist}, the waiting time $T$ for the next coalescence event (last coalescence at $t_0$ into $b$ lineages) fulfills 

$$P_{t_0}(T\leq t)=1-e^{\lambda_b(\rho\gamma)^{-1}(e^{\rho\gamma (t+t_0)}-e^{\rho\gamma t_0})}=1-e^{\lambda_b(\rho\gamma)^{-1}e^{\rho\gamma t_0}/e^{\rho\gamma t}-1}.$$ This is the distribution function of a Gompertz distribution with parameters $a=\lambda_be^{\rho\gamma t_0}$ and $b=\rho\gamma$, see e.g. \citet[Eq. 3]{lenart2014moments}.\\ 
The case of the (non-thinned) modified Moran models from the last section leading to Beta$(2,b)$-$n$-coalescents is excluded here, this case is covered later in Remark \ref{rem:cNeqlog}.  
\begin{remark}\label{rem:timechanges1}
The function $\mathcal{G}(t)$ depends on both $\rho$ and $\nu(t)$, so both on the amount of discrete generations corresponding to a unit of coalescent time and on the population size changes on the coalescent time scale. Especially for exponential size changes, $\mathcal{G}$ depends on the product $\gamma\rho$. This has been already discussed in \citep{Matuszewski2017}, where the problem of inference was highlighted: If one wants to infer $\rho$ directly (instead of the compound parameter $\rho\gamma$), $\gamma$ has to be known. This means that specifying/identifying the Cannings model leading to the limit process would be necessary to directly estimate $\rho$. This is very similar to the effect that e.g. Watterson's  estimator only allows to estimate the mutation rate on the coalescent time scale, and not the mutation rate in on generation, see e.g. \citet[p. 2627]{Eldon2006}.\\
As an example, consider the two sequences of modified Moran models leading to a (time-changed) Dirac $n$-coalescent from Remarks \ref{rem:diffmodMoran}: For a given $\nu$, their limits coincide if one uses the same order $N^{-\gamma}$ of $c_N$ for both models. However, even in each model series itself, changing $\gamma$ changes the time change function $\mathcal{G}(t)$, unless $\mathcal{G}(t)\equiv 1$ (which corresponds to the fixed-$N$ setting). Another example are the Wright-Fisher model and the (usual) Moran models. It is well known, see e.g. \cite{griffiths1994sampling}, that the rescaled genealogy of a sample from a Wright-Fisher model with asymtotically fluctuating population sizes described by $\nu$ converges to Kingman's $n$-coalescent with time change $\mathcal{G}$ as in Eq. \eqref{eq:compute_mathcalG} with $\gamma=1$. However, for the classic Moran model, $c_N=\frac{2}{N(N-1)}$ and Proposition \ref{lem:3Mconv} is applicable with allocation scheme $(\mathcal{RM})$, so  Eq. \eqref{eq:compute_mathcalG} holds with $\gamma=2$. For further discussion of this issue, see Remark \ref{rem:cNeqlog}. 
\end{remark}

 
\section{Sampling from super-critical branching with fluctuating population sizes}\label{sec:supercrit}
For Beta$(2-\alpha,\alpha)$-$n$-coalescents, $1\leq\alpha<2$, genealogies sampled from the fixed-$N$ Cannings models introduced in \cite{Schweinsberg2003} also converge weakly to these processes (after rescaling of time) for $N\to\infty$. They have been proposed as a model of type-III survivorship, where all individuals produce many offspring with a high juvenile mortality, see e.g. \citet[Sect. 2.3]{Steinruecken2013}.\\
This model (for fixed population size $N$) lets each individual in any generation $r$ produce a number of (potential) offspring $X^{(r)}_i$, i.i.d. across individuals and generations, distributed as a tail-heavy random variable $X$ with $E(X)=\mu>1$, i.e. $P(X\geq k)\sim Ck^{-\alpha}$ on $\mathbb{N}$  ($C>0$ constant, $1<\alpha<2$) and then $N$ offspring are chosen to form the next generation. If less than $N$ offspring are produced, the missing next generation individuals are arbitrarily associated with parents. Here, this is done by randomly choosing a parent, which preserves exchangeability and makes the model a Cannings model. The genealogies of a sample of size $n$ converge for $N\to\infty$ and time rescaled by $c_N^{-1}$ to the Beta($2-\alpha$,$\alpha$)-$n$-coalescent, see \citet[Thm. 4]{Schweinsberg2003}. \\
This model is extended by allowing population size changes as in \eqref{eq:cond_popsize}. Sampling fewer individuals than in total in the last generation is well-defined, but when individuals are added, it needs to be explained which parents they have. The supercritical branching produces, with very high probability, enough offspring so that one can just sample from the produced offspring and cover instantaneous expansions plus exponential size changes. This is shown in the following  
\begin{lemma}\label{lem:popsizechange_schwein}
Let $d_{N,r}:=N_{r-1}-N_r=s_{N,r}N_r>0$. Assume that for a fixed $t$ all $r\leq c^{-1}_Nt$ for any $t$  with a null sequence $(d_N)_{N\in\N}$ with $s_{N,r}\leq d_N$ for $N\to\infty$. Then, $P(\sum_i^{N_r} X_{(r)}^{i}<N_{r-1})\leq A^{N}$ with $N=N_0$.
\end{lemma}
\begin{proof}
It suffices to reiterate the proof of \citet[Lemma 5]{Schweinsberg2003} briefly. For $u\in[0,1]$, consider the generating function $f(u):=E(u^X)$. Then,  $S_{N,r}:=\sum_{i=1}^{N_r} X^{(r)}_i$ fulfills

$$P(S_{N,r}\leq N_{r-1})\leq u^{-N_r(1+s_{N,r})}E(u^{S_{N,r}})=(u^{-(1+s_{N,r})}f(u))^{N_r}.$$ Since $f(1)=1$ and $f'(1)=\mu>1$, there exists $u_0\in(0,1)$ and $\epsilon>0$ so that $u_0^{1+\epsilon}<f(u_0)$. Moreover, for this $\epsilon$ we find $N_0\in\N$ so that $d_N<\epsilon$ for $N\geq N_0$. For such $N$, as computed above, one gets 

$$P(S_{N,r}\leq N_{r-1})\leq (u_0^{-(1+s_{N,r})}f(u_0))^{N_r}\leq A_1^{N_r} \leq A_1^{N^{-}(t)}=(\underbrace{A_1^{c^{-}(t)}}_{<1})^N,$$
where $A_1:=u_0^{-(1+\epsilon)}f(u_0)<1$. Setting $A:=A_1^{c^{-}(t)}$ completes the proof.
\end{proof}  
For applying Lemma \ref{lem:cannpopsizetolambda}, assume that $|s_{N_r}|\leq d_N\to 0$ for any $r$, not only if $s_{N,r}>0$. Still, as in the case of modified Moran models, this allows both for instantaneous and exponential population size changes. Indeed, setting $N_{r+1}=(1-c_N\rho)N_r$ for units of coalescent time leads to exponential change in this timespan and fulfills $|s_{N_r}|\leq (1+\epsilon) c_N|\rho|=:d_N\to 0$ for an arbitrary $\epsilon>0$ and $N\to\infty$. For (coalescent time) instantaneous population size changes, i.e. for a size change of $d_{N,r}=mN$, use e.g. $|s_{N,r}|=m\sqrt{c_N}=:d_N\to 0$ for $N\to\infty$ for $(\sqrt{c_N})^{-1}$ generations.\\
Recall that, for $1<\alpha<2$, the coalescence probability in this (fixed-$N$) model satisfies $c_N\sim C\alpha B(2-\alpha,\alpha)E(X)^{-\alpha}N^{1-\alpha}$, where $B$ is the Beta function, see \citet[Lemma 13]{Schweinsberg2003}. For $\alpha=1$, instead $c_N\sim (\log N)^{-1}$, see \citet[Lemma 16]{Schweinsberg2003}.
\begin{proposition}\label{prop:schweinspopsized}
Consider the Cannings model coming from sampling from supercritical branching with parameter $\alpha\in[1,2)$ and variable population sizes $(N_r)_{r\in\N_0}$ and $N_0=N$. If $(N_r)_{r\in\N_0}$ fulfill \eqref{eq:cond_popsize} and $s_{N,r}=N_r^{-1}(N_{r-1}-N_r)\leq d_N\to 0$ for $N\to\infty$, then the discrete $n$-coalescents
$(\mathcal{R}_{G_N^{-1}(t)})_{t\geq 0}\stackrel{d}{\to}(\Pi_t)_{t\geq 0}$ in the Skorohod-sense, where $(\Pi_t)_{t\geq 0}$ is the Beta($2-\alpha,\alpha$)-$n$-coalescent. Equivalently, if we have $N^{-1}N_{\lfloor tc_N^{-1}\rfloor +1}\to \nu(t)>0$ for all $t$,   
 $(\mathcal{R}_{c_N^{-1}t})_{t\geq 0}\stackrel{d}{\to}(\Pi_{\mathcal{G}(t)})_{t\geq 0}$ in the Skorohod-sense, where $\mathcal{G}(t)=\int^t_0 (\nu(s))^{1-\alpha} ds$.
\end{proposition} 

\begin{proof} 
Check the conditions necessary to apply Lemma \ref{lem:cannpopsizetolambda}: The model and the assumptions above satisfy $c_N\to 0$, \eqref{eq:cond_popsize} and, since $c_N$ is regularly varying, also \eqref{eq:cond_speed_cN}. Thus, only \eqref{eq:cond_phi} needs to be verified. Since $N_{r-1}$ offspring are sampled from $\sum_{i=1}^{N_r}\nu^{(N_r)}_{i}$ potential offspring, 

\begin{align*}
\Phi^{(N)}(r;a_1,\ldots,a_l)=&\frac{E\left(\prod_{i=1}^l (\nu_i^{(N_r)})_{a_i}\right)}{\prod_{i=1}^l(N_{r-1})_{a_i}}=\Phi^{(N_r)}(a_1,\ldots,a_l)\frac{\prod_{i=1}^l(N_r)_{a_i}}{\prod_{i=1}^l(N_{r-1})_{a_i}}
\end{align*} 
This means one just needs to show that 

$$\Phi^{(N_r)}(a_1,\ldots,a_l)\left|\frac{\prod_{i=1}^l(N_r)_{a_i}}{\prod_{i=1}^l(N_{r-1})_{a_i}}-1\right|=o_{\sum}(c_N),$$ which follows from $c_N^{-1}\Phi^{(N_r)}(a_1,\ldots,a_l)\left|\frac{\prod_{i=1}^l(N_r)_{a_i}}{\prod_{i=1}^l(N_{r-1})_{a_i}}-1\right|\to 0$ uniformly in $r$. To show this, first observe that, since \eqref{eq:cond_speed_cN} holds, 

$$c_N^{-1}\Phi^{(N_r)}(a_1,\ldots,a_l)=\underbrace{c_{N_r}^{-1}\Phi^{(N_r)}(a_1,\ldots,a_l)}_{\to \phi(a_1,\ldots,a_l)}\frac{c_{N_r}}{c_N}$$ is uniformly bounded (again, since $N_r$ is bounded from below by $N^-(t)$, there is uniform convergence in $r$ of the first factor for $N\to\infty$). Thus, we only need to show $\left|\frac{\prod_{i=1}^l(N_r)_{a_i}}{\prod_{i=1}^l(N_{r-1})_{a_i}}-1\right|\to 0$. For this, observe that the function $x\mapsto\frac{a_1-x}{a_2-x}$ for $x<a_2$ is strictly increasing (decreasing) if $a_1-a_2>0$ (if $a_1-a_2<0$). This shows that there are $b_1,b_2\in\N_0$ so that 

$$\left(\frac{N_r-b_1}{N_{r-1}-b_1}\right)^{\sum_i^l a_i}\leq\frac{\prod_{i=1}^l(N_r)_{a_i}}{\prod_{i=1}^l(N_{r-1})_{a_i}}\leq\left(\frac{N_r-b_2}{N_{r-1}-b_2}\right)^{\sum_i^l a_i}.$$ This implies that it is sufficient to show $\left|\left(\frac{N_r-b}{N_{r-1}-b}\right)^{\sum_i^l a_i}-1\right|\to 0$ for any $N^-(t)>b\geq 0$. For any sequence $(x_{N,r})_{N,r}$,

$$x_{N,r}\to 1 \Rightarrow |x^{k}_{N,r}-1|=|(x_{N,r}-1)\sum_{i=0}^{k-1} x_{N,r}^{i}|\to 0$$ for $k\in\N$ if $\sum_{i=0}^{k-1} x_{N,r}^{i}$ is uniformly bounded for $N,r$. This is satisfied for $x_{N,r}=\frac{N_r-b}{N_{r-1}-b}\leq \frac{N^+(t)-b}{N^{-}(t)-b}$, so it is sufficient to show $\left|\left(\frac{N_r-b}{N_{r-1}-b}\right)-1\right|\to 0$ uniformly in $r$. 
Further computation shows

$$
\left|\frac{N_r-b}{N_{r-1}-b}-1\right|=\frac{|d_{N,r}|}{N_{r-1}-b}\leq \frac{d_N}{N_{r-1}-b}.   
$$
Since $d_N\to 0$, this vanishes uniformly. Thus, Lemma \ref{lem:cannpopsizetolambda} can be applied, establishing convergence of  $(\mathcal{R}_{G_N^{-1}(t)})_{t\geq 0}\stackrel{d}{\to}(\Pi_{t})_{t\geq 0}$. To replace the scaling function $G_N$ by scaling with $c_N^{-1}$, this works analogously to Section \ref{sec:scaletolim} if $\alpha>1$, just set $\gamma=\alpha-1$. For $\alpha=1$,  the proofs of that section need to be adapted slightly. First, Eq. \eqref{eq:compute_mathcalG} still holds. We have $c_N=\log N + o_{\sum}(c_N)$, so for computing $F_N$ and subsequently $\mathcal{G}$, one can again omit all $o$-terms and use $\log(N_r)^{-1}$ instead of $c_{N,r}$. Thus, using $k_r$ defined by $N_r=Nk_r$ for $0\leq r \leq c_{N}^{-1}t$  with $c_1(t)\leq k_r\leq c_2(t)$, 

\begin{align*}
\mathcal{G}(t)=&\lim_{N\to\infty}\sum_{r=1}^{[tc_{N}^{-1}]}\log(N)^{-1}\frac{\log(N)}{\log(N_r)}\\=&\lim_{N\to\infty}\sum_{r=1}^{[t\log(N)]}\log(N)^{-1}\left(1-\frac{k_r}{\log(N)+k_r}\right)\\
=& t-\lim_{N\to\infty}\sum_{r=1}^{[t\log(N)]}\frac{k_r}{(\log(N)+k_r)\log(N)}=t=\int_0^t (\nu(s))^0 ds.
\end{align*}
 \end{proof}
\begin{remark}\label{rem:cNeqlog}
For $\alpha=1$ in Proposition \ref{prop:schweinspopsized}, the time change is given by $\mathcal{G}(t)=t$, regardless of the actual population size changes $\nu$ on the coalescent time scale. Thus, for $\alpha=1$ population size changes of order $N$ on the coalescent time scale have no influence on the genealogy, which in this case always is the Bolthausen-Sznitman $n$-coalescent. However, if for the Cannings models, one chooses the modified Moran models introduced above with the same fixed-$N$ limit genealogy tree, i.e. the Bolthausen-Sznitman $n$-coalescent, and with the same population size changes $\nu(t)$ on the coalescent time scale, $\mathcal{G}$ is affected by the specific choice of $\nu$. This again highlights that the limit genealogy is strongly affected by both $\nu$ and the discrete Cannings models used for construction (i.e. $c_N$ of the latter).
Interestingly, the exact same behaviour happens for the modified Moran models used earlier to construct Beta($2$,b)-$n$-coalescents. There $c_N$ is again of order $\log(N)^{-1}$. The limit genealogy of $n$ individuals sampled from these modified Moran models including any population size changes allowed in Proposition \ref{lem:3Mconv} (e.g. exponential growth and any population decline) will always be the non-rescaled Beta$(2,b)$-$n$-coalescent. 
\end{remark}
\section{Discussion}\label{sec:disc}
As for the Wright-Fisher model, genealogies of samples taken from many families of (haploid) modified Moran and other Cannings models can be approximated by a time-change of their (multiple-merger) limit coalescent process, when the population sizes of the discrete models are fluctuating, but are always of the same order of size. As for models with fixed population size, times measured in an unit of $c^{-1}_N$ generations in the discrete model correspond to a unit of size 1 in the continuous time limit.
\\ The modified Moran models used to construct the time-changed $\Lambda$-$n$-coalescents can be described as follows (approximately for $N\to\infty$): Either in every generation or occasionally (in the latter switching to a normal Moran model if this does not happen), there is a (possibly random) probability $p$ for each individual to not have offspring in the next generation. From the individuals that have offspring, all but one reproduce once, and one individual replaces itself and all non-reproducing individuals by its offspring. These models capture the concept of sweepstake reproduction \citep{Hedgecock2011}, though the assumption of a single individual with more than one offspring is rather artificial. However, these are just one possible choice of modified Moran, or more general Cannings, models that lead to a specific time-changed $\Lambda$-$n$-coalescent. For instance, if the population is modelled by sampling the next generation from a supercritical branching process with heavy-tailed offspring distribution, this again leads to a (time-changed) Beta-$n$-coalescent limit.\\
It should be stressed that both the profile of population size changes and the coalescence probabilities $c_N$ affect the time change of the limit coalescent for population size $N\to\infty$. Even if two sequences of discrete models lead, when population size $N$ is constant across generations, to the same limit when genealogies are rescaled by $c^{-1}_N$, adding the same population size changes in both models on the coalescent time scale can lead to different time scalings of the limit. This shows that for inference of the population size changes, the discrete reproduction models need to be specified or its effects may not be disentangled from the population size changes.\\
For some families of Cannings models, if the coalescence probability $c_N$ is of order $\log(N)^{-1}$, which is relatively high, population size changes of order $N$ may not even alter the limit genealogy. On this scale, coalescence probabilities are not altered meaningfully by non-extreme population size changes.\\
  While the results cover the Bolthausen-Sznitman $n$-coalescent ($\Lambda=$Beta$(1,1)$) with population size changes as a possible limit model, the discrete models used to explicitly construct it are not based on modelling of a directed selection process due to selective advantages of certain ancestral lineages. Thus, the results do not answer whether adding population size changes to a model of rapid selection or genetic draft as in \cite{Desai2013,Neher2013a,Schweinsberg2017} also leads to its rescaled genealogies being described by a time-rescaled Bolthausen-Sznitman $n$-coalescent.  
